The Shapes of Tight Composite Knots

We present new computations of tight shapes obtained using the constrained gradient descent code RIDGERUNNER for 544 composite knots with 12 and fewer crossings, expanding our dataset to 943 knots and links. We use the new data set to analyze two outstanding conjectures about tight knots, namely that the ropelengths of composite knots are at least 4\pi-4 less than the sums of the prime factors and that the writhes of composite knots are the sums of the writhes of the prime factors.

==> latex_knot_impr.tex <==
\newcommand{ \TwoTwoOneImpr }{-}

\FPeval{\ThreeOneImpr}{100.0*((\ThreeOnePrev - \ThreeOneRRUB)/(\ThreeOnePrev))}
\FPround{\ThreeOneImpr}{\ThreeOneImpr}{2}
\FPeval{\FourOneImpr}{100.0*((\FourOnePrev - \FourOneRRUB)/(\FourOnePrev))}
\FPround{\FourOneImpr}{\FourOneImpr}{2}
\newcommand{ \FourTwoOneImpr }{-}

\FPeval{\FiveOneImpr}{100.0*((\FiveOnePrev - \FiveOneRRUB)/(\FiveOnePrev))}
\FPround{\FiveOneImpr}{\FiveOneImpr}{2}
\newcommand{ \FiveTwoOneImpr }{-}

\FPeval{\FiveTwoImpr}{100.0*((\FiveTwoPrev - \FiveTwoRRUB)/(\FiveTwoPrev))}
\FPround{\FiveTwoImpr}{\FiveTwoImpr}{2}
\FPeval{\SixOneImpr}{100.0*((\SixOnePrev - \SixOneRRUB)/(\SixOnePrev))}
\FPround{\SixOneImpr}{\SixOneImpr}{2}
\newcommand{ \SixTwoOneImpr }{-}

\newcommand{ \SixTwoTwoImpr }{-}

\newcommand{ \SixTwoThreeImpr }{-}

\FPeval{\SixTwoImpr}{100.0*((\SixTwoPrev - \SixTwoRRUB)/(\SixTwoPrev))}
\FPround{\SixTwoImpr}{\SixTwoImpr}{2}
\newcommand{ \SixThreeOneImpr }{-}

\newcommand{ \SixThreeTwoImpr }{-}

\newcommand{ \SixThreeThreeImpr }{-}

\FPeval{\SixThreeImpr}{100.0*((\SixThreePrev - \SixThreeRRUB)/(\SixThreePrev))}
\FPround{\SixThreeImpr}{\SixThreeImpr}{2}
\FPeval{\SevenOneImpr}{100.0*((\SevenOnePrev - \SevenOneRRUB)/(\SevenOnePrev))}
\FPround{\SevenOneImpr}{\SevenOneImpr}{2}
\newcommand{ \SevenTwoOneImpr }{-}

\newcommand{ \SevenTwoTwoImpr }{-}

\newcommand{ \SevenTwoThreeImpr }{-}

\newcommand{ \SevenTwoFourImpr }{-}

\newcommand{ \SevenTwoFiveImpr }{-}

\newcommand{ \SevenTwoSixImpr }{-}

\newcommand{ \SevenTwoSevenImpr }{-}

\newcommand{ \SevenTwoEightImpr }{-}

\FPeval{\SevenTwoImpr}{100.0*((\SevenTwoPrev - \SevenTwoRRUB)/(\SevenTwoPrev))}
\FPround{\SevenTwoImpr}{\SevenTwoImpr}{2}
\newcommand{ \SevenThreeOneImpr }{-}

\FPeval{\SevenThreeImpr}{100.0*((\SevenThreePrev - \SevenThreeRRUB)/(\SevenThreePrev))}
\FPround{\SevenThreeImpr}{\SevenThreeImpr}{2}
\FPeval{\SevenFourImpr}{100.0*((\SevenFourPrev - \SevenFourRRUB)/(\SevenFourPrev))}
\FPround{\SevenFourImpr}{\SevenFourImpr}{2}
\FPeval{\SevenFiveImpr}{100.0*((\SevenFivePrev - \SevenFiveRRUB)/(\SevenFivePrev))}
\FPround{\SevenFiveImpr}{\SevenFiveImpr}{2}
\FPeval{\SevenSixImpr}{100.0*((\SevenSixPrev - \SevenSixRRUB)/(\SevenSixPrev))}
\FPround{\SevenSixImpr}{\SevenSixImpr}{2}
\FPeval{\SevenSevenImpr}{100.0*((\SevenSevenPrev - \SevenSevenRRUB)/(\SevenSevenPrev))}
\FPround{\SevenSevenImpr}{\SevenSevenImpr}{2}
\FPeval{\EightOneImpr}{100.0*((\EightOnePrev - \EightOneRRUB)/(\EightOnePrev))}
\FPround{\EightOneImpr}{\EightOneImpr}{2}
\FPeval{\EightTenImpr}{100.0*((\EightTenPrev - \EightTenRRUB)/(\EightTenPrev))}
\FPround{\EightTenImpr}{\EightTenImpr}{2}
\FPeval{\EightElevenImpr}{100.0*((\EightElevenPrev - \EightElevenRRUB)/(\EightElevenPrev))}
\FPround{\EightElevenImpr}{\EightElevenImpr}{2}
\FPeval{\EightTwelveImpr}{100.0*((\EightTwelvePrev - \EightTwelveRRUB)/(\EightTwelvePrev))}
\FPround{\EightTwelveImpr}{\EightTwelveImpr}{2}
\FPeval{\EightThirteenImpr}{100.0*((\EightThirteenPrev - \EightThirteenRRUB)/(\EightThirteenPrev))}
\FPround{\EightThirteenImpr}{\EightThirteenImpr}{2}
\FPeval{\EightFourteenImpr}{100.0*((\EightFourteenPrev - \EightFourteenRRUB)/(\EightFourteenPrev))}
\FPround{\EightFourteenImpr}{\EightFourteenImpr}{2}
\FPeval{\EightFifteenImpr}{100.0*((\EightFifteenPrev - \EightFifteenRRUB)/(\EightFifteenPrev))}
\FPround{\EightFifteenImpr}{\EightFifteenImpr}{2}
\FPeval{\EightSixteenImpr}{100.0*((\EightSixteenPrev - \EightSixteenRRUB)/(\EightSixteenPrev))}
\FPround{\EightSixteenImpr}{\EightSixteenImpr}{2}
\FPeval{\EightSeventeenImpr}{100.0*((\EightSeventeenPrev - \EightSeventeenRRUB)/(\EightSeventeenPrev))}
\FPround{\EightSeventeenImpr}{\EightSeventeenImpr}{2}
\FPeval{\EightEighteenImpr}{100.0*((\EightEighteenPrev - \EightEighteenRRUB)/(\EightEighteenPrev))}
\FPround{\EightEighteenImpr}{\EightEighteenImpr}{2}
\FPeval{\EightNineteenImpr}{100.0*((\EightNineteenPrev - \EightNineteenRRUB)/(\EightNineteenPrev))}
\FPround{\EightNineteenImpr}{\EightNineteenImpr}{2}
\newcommand{ \EightTwoOneImpr }{-}

\newcommand{ \EightTwoTenImpr }{-}

\newcommand{ \EightTwoElevenImpr }{-}

\newcommand{ \EightTwoTwelveImpr }{-}

\newcommand{ \EightTwoThirteenImpr }{-}

\newcommand{ \EightTwoFourteenImpr }{-}

\newcommand{ \EightTwoFifteenImpr }{-}

\newcommand{ \EightTwoSixteenImpr }{-}

\newcommand{ \EightTwoTwoImpr }{-}

\newcommand{ \EightTwoThreeImpr }{-}

\newcommand{ \EightTwoFourImpr }{-}

\newcommand{ \EightTwoFiveImpr }{-}

\newcommand{ \EightTwoSixImpr }{-}

\newcommand{ \EightTwoSevenImpr }{-}

\newcommand{ \EightTwoEightImpr }{-}

\newcommand{ \EightTwoNineImpr }{-}

\FPeval{\EightTwoImpr}{100.0*((\EightTwoPrev - \EightTwoRRUB)/(\EightTwoPrev))}
\FPround{\EightTwoImpr}{\EightTwoImpr}{2}
\FPeval{\EightTwentyImpr}{100.0*((\EightTwentyPrev - \EightTwentyRRUB)/(\EightTwentyPrev))}
\FPround{\EightTwentyImpr}{\EightTwentyImpr}{2}
\FPeval{\EightTwentyoneImpr}{100.0*((\EightTwentyonePrev - \EightTwentyoneRRUB)/(\EightTwentyonePrev))}
\FPround{\EightTwentyoneImpr}{\EightTwentyoneImpr}{2}
\newcommand{ \EightThreeOneImpr }{-}

\newcommand{ \EightThreeTenImpr }{-}

\newcommand{ \EightThreeTwoImpr }{-}

\newcommand{ \EightThreeThreeImpr }{-}

\newcommand{ \EightThreeFourImpr }{-}

\newcommand{ \EightThreeFiveImpr }{-}

\newcommand{ \EightThreeSixImpr }{-}

\newcommand{ \EightThreeSevenImpr }{-}

\newcommand{ \EightThreeEightImpr }{-}

\newcommand{ \EightThreeNineImpr }{-}

\FPeval{\EightThreeImpr}{100.0*((\EightThreePrev - \EightThreeRRUB)/(\EightThreePrev))}
\FPround{\EightThreeImpr}{\EightThreeImpr}{2}
\newcommand{ \EightFourOneImpr }{-}

\newcommand{ \EightFourTwoImpr }{-}

\newcommand{ \EightFourThreeImpr }{-}

\FPeval{\EightFourImpr}{100.0*((\EightFourPrev - \EightFourRRUB)/(\EightFourPrev))}
\FPround{\EightFourImpr}{\EightFourImpr}{2}
\FPeval{\EightFiveImpr}{100.0*((\EightFivePrev - \EightFiveRRUB)/(\EightFivePrev))}
\FPround{\EightFiveImpr}{\EightFiveImpr}{2}
\FPeval{\EightSixImpr}{100.0*((\EightSixPrev - \EightSixRRUB)/(\EightSixPrev))}
\FPround{\EightSixImpr}{\EightSixImpr}{2}
\FPeval{\EightSevenImpr}{100.0*((\EightSevenPrev - \EightSevenRRUB)/(\EightSevenPrev))}
\FPround{\EightSevenImpr}{\EightSevenImpr}{2}
\FPeval{\EightEightImpr}{100.0*((\EightEightPrev - \EightEightRRUB)/(\EightEightPrev))}
\FPround{\EightEightImpr}{\EightEightImpr}{2}
\FPeval{\EightNineImpr}{100.0*((\EightNinePrev - \EightNineRRUB)/(\EightNinePrev))}
\FPround{\EightNineImpr}{\EightNineImpr}{2}
\FPeval{\NineOneImpr}{100.0*((\NineOnePrev - \NineOneRRUB)/(\NineOnePrev))}
\FPround{\NineOneImpr}{\NineOneImpr}{2}
\FPeval{\NineTenImpr}{100.0*((\NineTenPrev - \NineTenRRUB)/(\NineTenPrev))}
\FPround{\NineTenImpr}{\NineTenImpr}{2}
\FPeval{\NineElevenImpr}{100.0*((\NineElevenPrev - \NineElevenRRUB)/(\NineElevenPrev))}
\FPround{\NineElevenImpr}{\NineElevenImpr}{2}
\FPeval{\NineTwelveImpr}{100.0*((\NineTwelvePrev - \NineTwelveRRUB)/(\NineTwelvePrev))}
\FPround{\NineTwelveImpr}{\NineTwelveImpr}{2}
\FPeval{\NineThirteenImpr}{100.0*((\NineThirteenPrev - \NineThirteenRRUB)/(\NineThirteenPrev))}
\FPround{\NineThirteenImpr}{\NineThirteenImpr}{2}
\FPeval{\NineFourteenImpr}{100.0*((\NineFourteenPrev - \NineFourteenRRUB)/(\NineFourteenPrev))}
\FPround{\NineFourteenImpr}{\NineFourteenImpr}{2}
\FPeval{\NineFifteenImpr}{100.0*((\NineFifteenPrev - \NineFifteenRRUB)/(\NineFifteenPrev))}
\FPround{\NineFifteenImpr}{\NineFifteenImpr}{2}
\FPeval{\NineSixteenImpr}{100.0*((\NineSixteenPrev - \NineSixteenRRUB)/(\NineSixteenPrev))}
\FPround{\NineSixteenImpr}{\NineSixteenImpr}{2}
\FPeval{\NineSeventeenImpr}{100.0*((\NineSeventeenPrev - \NineSeventeenRRUB)/(\NineSeventeenPrev))}
\FPround{\NineSeventeenImpr}{\NineSeventeenImpr}{2}
\FPeval{\NineEighteenImpr}{100.0*((\NineEighteenPrev - \NineEighteenRRUB)/(\NineEighteenPrev))}
\FPround{\NineEighteenImpr}{\NineEighteenImpr}{2}
\FPeval{\NineNineteenImpr}{100.0*((\NineNineteenPrev - \NineNineteenRRUB)/(\NineNineteenPrev))}
\FPround{\NineNineteenImpr}{\NineNineteenImpr}{2}
\newcommand{ \NineTwoOneImpr }{-}

\newcommand{ \NineTwoTenImpr }{-}

\newcommand{ \NineTwoElevenImpr }{-}

\newcommand{ \NineTwoTwelveImpr }{-}

\newcommand{ \NineTwoThirteenImpr }{-}

\newcommand{ \NineTwoFourteenImpr }{-}

\newcommand{ \NineTwoFifteenImpr }{-}

\newcommand{ \NineTwoSixteenImpr }{-}

\newcommand{ \NineTwoSeventeenImpr }{-}

\newcommand{ \NineTwoEighteenImpr }{-}

\newcommand{ \NineTwoNineteenImpr }{-}

\newcommand{ \NineTwoTwoImpr }{-}

\newcommand{ \NineTwoTwentyImpr }{-}

\newcommand{ \NineTwoTwentyoneImpr }{-}

\newcommand{ \NineTwoTwentytwoImpr }{-}

\newcommand{ \NineTwoTwentythreeImpr }{-}

\newcommand{ \NineTwoTwentyfourImpr }{-}

\newcommand{ \NineTwoTwentyfiveImpr }{-}

\newcommand{ \NineTwoTwentysixImpr }{-}

\newcommand{ \NineTwoTwentysevenImpr }{-}

\newcommand{ \NineTwoTwentyeightImpr }{-}

\newcommand{ \NineTwoTwentynineImpr }{-}

\newcommand{ \NineTwoThreeImpr }{-}

\newcommand{ \NineTwoThirtyImpr }{-}

\newcommand{ \NineTwoThirtyoneImpr }{-}

\newcommand{ \NineTwoThirtytwoImpr }{-}

\newcommand{ \NineTwoThirtythreeImpr }{-}

\newcommand{ \NineTwoThirtyfourImpr }{-}

\newcommand{ \NineTwoThirtyfiveImpr }{-}

\newcommand{ \NineTwoThirtysixImpr }{-}

\newcommand{ \NineTwoThirtysevenImpr }{-}

\newcommand{ \NineTwoThirtyeightImpr }{-}

\newcommand{ \NineTwoThirtynineImpr }{-}

\newcommand{ \NineTwoFourImpr }{-}

\newcommand{ \NineTwoFortyImpr }{-}

\newcommand{ \NineTwoFortyoneImpr }{-}

\newcommand{ \NineTwoFortytwoImpr }{-}

\newcommand{ \NineTwoFortythreeImpr }{-}

\newcommand{ \NineTwoFortyfourImpr }{-}

\newcommand{ \NineTwoFortyfiveImpr }{-}

\newcommand{ \NineTwoFortysixImpr }{-}

\newcommand{ \NineTwoFortysevenImpr }{-}

\newcommand{ \NineTwoFortyeightImpr }{-}

\newcommand{ \NineTwoFortynineImpr }{-}

\newcommand{ \NineTwoFiveImpr }{-}

\newcommand{ \NineTwoFiftyImpr }{-}

\newcommand{ \NineTwoFiftyoneImpr }{-}

\newcommand{ \NineTwoFiftytwoImpr }{-}

\newcommand{ \NineTwoFiftythreeImpr }{-}

\newcommand{ \NineTwoFiftyfourImpr }{-}

\newcommand{ \NineTwoFiftyfiveImpr }{-}

\newcommand{ \NineTwoFiftysixImpr }{-}

\newcommand{ \NineTwoFiftysevenImpr }{-}

\newcommand{ \NineTwoFiftyeightImpr }{-}

\newcommand{ \NineTwoFiftynineImpr }{-}

\newcommand{ \NineTwoSixImpr }{-}

\newcommand{ \NineTwoSixtyImpr }{-}

\newcommand{ \NineTwoSixtyoneImpr }{-}

\newcommand{ \NineTwoSevenImpr }{-}

\newcommand{ \NineTwoEightImpr }{-}

\newcommand{ \NineTwoNineImpr }{-}

\FPeval{\NineTwoImpr}{100.0*((\NineTwoPrev - \NineTwoRRUB)/(\NineTwoPrev))}
\FPround{\NineTwoImpr}{\NineTwoImpr}{2}
\FPeval{\NineTwentyImpr}{100.0*((\NineTwentyPrev - \NineTwentyRRUB)/(\NineTwentyPrev))}
\FPround{\NineTwentyImpr}{\NineTwentyImpr}{2}
\FPeval{\NineTwentyoneImpr}{100.0*((\NineTwentyonePrev - \NineTwentyoneRRUB)/(\NineTwentyonePrev))}
\FPround{\NineTwentyoneImpr}{\NineTwentyoneImpr}{2}
\FPeval{\NineTwentytwoImpr}{100.0*((\NineTwentytwoPrev - \NineTwentytwoRRUB)/(\NineTwentytwoPrev))}
\FPround{\NineTwentytwoImpr}{\NineTwentytwoImpr}{2}
\FPeval{\NineTwentythreeImpr}{100.0*((\NineTwentythreePrev - \NineTwentythreeRRUB)/(\NineTwentythreePrev))}
\FPround{\NineTwentythreeImpr}{\NineTwentythreeImpr}{2}
\FPeval{\NineTwentyfourImpr}{100.0*((\NineTwentyfourPrev - \NineTwentyfourRRUB)/(\NineTwentyfourPrev))}
\FPround{\NineTwentyfourImpr}{\NineTwentyfourImpr}{2}
\FPeval{\NineTwentyfiveImpr}{100.0*((\NineTwentyfivePrev - \NineTwentyfiveRRUB)/(\NineTwentyfivePrev))}
\FPround{\NineTwentyfiveImpr}{\NineTwentyfiveImpr}{2}
\FPeval{\NineTwentysixImpr}{100.0*((\NineTwentysixPrev - \NineTwentysixRRUB)/(\NineTwentysixPrev))}
\FPround{\NineTwentysixImpr}{\NineTwentysixImpr}{2}
\FPeval{\NineTwentysevenImpr}{100.0*((\NineTwentysevenPrev - \NineTwentysevenRRUB)/(\NineTwentysevenPrev))}
\FPround{\NineTwentysevenImpr}{\NineTwentysevenImpr}{2}
\FPeval{\NineTwentyeightImpr}{100.0*((\NineTwentyeightPrev - \NineTwentyeightRRUB)/(\NineTwentyeightPrev))}
\FPround{\NineTwentyeightImpr}{\NineTwentyeightImpr}{2}
\FPeval{\NineTwentynineImpr}{100.0*((\NineTwentyninePrev - \NineTwentynineRRUB)/(\NineTwentyninePrev))}
\FPround{\NineTwentynineImpr}{\NineTwentynineImpr}{2}
\newcommand{ \NineThreeOneImpr }{-}

\newcommand{ \NineThreeTenImpr }{-}

\newcommand{ \NineThreeElevenImpr }{-}

\newcommand{ \NineThreeTwelveImpr }{-}

\newcommand{ \NineThreeThirteenImpr }{-}

\newcommand{ \NineThreeFourteenImpr }{-}

\newcommand{ \NineThreeFifteenImpr }{-}

\newcommand{ \NineThreeSixteenImpr }{-}

\newcommand{ \NineThreeSeventeenImpr }{-}

\newcommand{ \NineThreeEighteenImpr }{-}

\newcommand{ \NineThreeNineteenImpr }{-}

\newcommand{ \NineThreeTwoImpr }{-}

\newcommand{ \NineThreeTwentyImpr }{-}

\newcommand{ \NineThreeTwentyoneImpr }{-}

\newcommand{ \NineThreeThreeImpr }{-}

\newcommand{ \NineThreeFourImpr }{-}

\newcommand{ \NineThreeFiveImpr }{-}

\newcommand{ \NineThreeSixImpr }{-}

\newcommand{ \NineThreeSevenImpr }{-}

\newcommand{ \NineThreeEightImpr }{-}

\newcommand{ \NineThreeNineImpr }{-}

\FPeval{\NineThreeImpr}{100.0*((\NineThreePrev - \NineThreeRRUB)/(\NineThreePrev))}
\FPround{\NineThreeImpr}{\NineThreeImpr}{2}
\FPeval{\NineThirtyImpr}{100.0*((\NineThirtyPrev - \NineThirtyRRUB)/(\NineThirtyPrev))}
\FPround{\NineThirtyImpr}{\NineThirtyImpr}{2}
\FPeval{\NineThirtyoneImpr}{100.0*((\NineThirtyonePrev - \NineThirtyoneRRUB)/(\NineThirtyonePrev))}
\FPround{\NineThirtyoneImpr}{\NineThirtyoneImpr}{2}
\FPeval{\NineThirtytwoImpr}{100.0*((\NineThirtytwoPrev - \NineThirtytwoRRUB)/(\NineThirtytwoPrev))}
\FPround{\NineThirtytwoImpr}{\NineThirtytwoImpr}{2}
\FPeval{\NineThirtythreeImpr}{100.0*((\NineThirtythreePrev - \NineThirtythreeRRUB)/(\NineThirtythreePrev))}
\FPround{\NineThirtythreeImpr}{\NineThirtythreeImpr}{2}
\FPeval{\NineThirtyfourImpr}{100.0*((\NineThirtyfourPrev - \NineThirtyfourRRUB)/(\NineThirtyfourPrev))}
\FPround{\NineThirtyfourImpr}{\NineThirtyfourImpr}{2}
\FPeval{\NineThirtyfiveImpr}{100.0*((\NineThirtyfivePrev - \NineThirtyfiveRRUB)/(\NineThirtyfivePrev))}
\FPround{\NineThirtyfiveImpr}{\NineThirtyfiveImpr}{2}
\FPeval{\NineThirtysixImpr}{100.0*((\NineThirtysixPrev - \NineThirtysixRRUB)/(\NineThirtysixPrev))}
\FPround{\NineThirtysixImpr}{\NineThirtysixImpr}{2}
\FPeval{\NineThirtysevenImpr}{100.0*((\NineThirtysevenPrev - \NineThirtysevenRRUB)/(\NineThirtysevenPrev))}
\FPround{\NineThirtysevenImpr}{\NineThirtysevenImpr}{2}
\FPeval{\NineThirtyeightImpr}{100.0*((\NineThirtyeightPrev - \NineThirtyeightRRUB)/(\NineThirtyeightPrev))}
\FPround{\NineThirtyeightImpr}{\NineThirtyeightImpr}{2}
\FPeval{\NineThirtynineImpr}{100.0*((\NineThirtyninePrev - \NineThirtynineRRUB)/(\NineThirtyninePrev))}
\FPround{\NineThirtynineImpr}{\NineThirtynineImpr}{2}
\newcommand{ \NineFourOneImpr }{-}

\FPeval{\NineFourImpr}{100.0*((\NineFourPrev - \NineFourRRUB)/(\NineFourPrev))}
\FPround{\NineFourImpr}{\NineFourImpr}{2}
\FPeval{\NineFortyImpr}{100.0*((\NineFortyPrev - \NineFortyRRUB)/(\NineFortyPrev))}
\FPround{\NineFortyImpr}{\NineFortyImpr}{2}
\FPeval{\NineFortyoneImpr}{100.0*((\NineFortyonePrev - \NineFortyoneRRUB)/(\NineFortyonePrev))}
\FPround{\NineFortyoneImpr}{\NineFortyoneImpr}{2}
\FPeval{\NineFortytwoImpr}{100.0*((\NineFortytwoPrev - \NineFortytwoRRUB)/(\NineFortytwoPrev))}
\FPround{\NineFortytwoImpr}{\NineFortytwoImpr}{2}
\FPeval{\NineFortythreeImpr}{100.0*((\NineFortythreePrev - \NineFortythreeRRUB)/(\NineFortythreePrev))}
\FPround{\NineFortythreeImpr}{\NineFortythreeImpr}{2}
\FPeval{\NineFortyfourImpr}{100.0*((\NineFortyfourPrev - \NineFortyfourRRUB)/(\NineFortyfourPrev))}
\FPround{\NineFortyfourImpr}{\NineFortyfourImpr}{2}
\FPeval{\NineFortyfiveImpr}{100.0*((\NineFortyfivePrev - \NineFortyfiveRRUB)/(\NineFortyfivePrev))}
\FPround{\NineFortyfiveImpr}{\NineFortyfiveImpr}{2}
\FPeval{\NineFortysixImpr}{100.0*((\NineFortysixPrev - \NineFortysixRRUB)/(\NineFortysixPrev))}
\FPround{\NineFortysixImpr}{\NineFortysixImpr}{2}
\FPeval{\NineFortysevenImpr}{100.0*((\NineFortysevenPrev - \NineFortysevenRRUB)/(\NineFortysevenPrev))}
\FPround{\NineFortysevenImpr}{\NineFortysevenImpr}{2}
\FPeval{\NineFortyeightImpr}{100.0*((\NineFortyeightPrev - \NineFortyeightRRUB)/(\NineFortyeightPrev))}
\FPround{\NineFortyeightImpr}{\NineFortyeightImpr}{2}
\FPeval{\NineFortynineImpr}{100.0*((\NineFortyninePrev - \NineFortynineRRUB)/(\NineFortyninePrev))}
\FPround{\NineFortynineImpr}{\NineFortynineImpr}{2}
\FPeval{\NineFiveImpr}{100.0*((\NineFivePrev - \NineFiveRRUB)/(\NineFivePrev))}
\FPround{\NineFiveImpr}{\NineFiveImpr}{2}
\FPeval{\NineSixImpr}{100.0*((\NineSixPrev - \NineSixRRUB)/(\NineSixPrev))}
\FPround{\NineSixImpr}{\NineSixImpr}{2}
\FPeval{\NineSevenImpr}{100.0*((\NineSevenPrev - \NineSevenRRUB)/(\NineSevenPrev))}
\FPround{\NineSevenImpr}{\NineSevenImpr}{2}
\FPeval{\NineEightImpr}{100.0*((\NineEightPrev - \NineEightRRUB)/(\NineEightPrev))}
\FPround{\NineEightImpr}{\NineEightImpr}{2}
\FPeval{\NineNineImpr}{100.0*((\NineNinePrev - \NineNineRRUB)/(\NineNinePrev))}
\FPround{\NineNineImpr}{\NineNineImpr}{2}


==> latex_knot_prop.tex <==
\newcommand{\TwoTwoOneRProp}{25.1439}
\newcommand{\ThreeOneRProp}{32.7490}
\newcommand{\FourOneRProp}{42.0997}
\newcommand{\FourTwoOneRProp}{40.0247}
\newcommand{\FiveOneRProp}{47.2156}
\newcommand{\FiveTwoOneRProp}{49.7874}
\newcommand{\FiveTwoRProp}{49.4840}
\newcommand{\SixOneRProp}{56.7316}
\newcommand{\SixTwoOneRProp}{54.4068}
\newcommand{\SixTwoTwoRProp}{56.7132}
\newcommand{\SixTwoThreeRProp}{58.1161}
\newcommand{\SixTwoRProp}{57.0451}
\newcommand{\SixThreeOneRProp}{57.8334}
\newcommand{\SixThreeTwoRProp}{58.0300}
\newcommand{\SixThreeThreeRProp}{50.5865}
\newcommand{\SixThreeRProp}{57.8602}
\newcommand{\SevenOneRProp}{61.4319}
\newcommand{\SevenTwoOneRProp}{64.2585}
\newcommand{\SevenTwoTwoRProp}{65.0467}
\newcommand{\SevenTwoThreeRProp}{65.3743}
\newcommand{\SevenTwoFourRProp}{65.0971}
\newcommand{\SevenTwoFiveRProp}{66.2400}
\newcommand{\SevenTwoSixRProp}{66.3494}
\newcommand{\SevenTwoSevenRProp}{55.5451}
\newcommand{\SevenTwoEightRProp}{57.8043}
\newcommand{\SevenTwoRProp}{63.9165}
\newcommand{\SevenThreeOneRProp}{65.8275}
\newcommand{\SevenThreeRProp}{63.9539}
\newcommand{\SevenFourRProp}{64.2960}
\newcommand{\SevenFiveRProp}{65.2802}
\newcommand{\SevenSixRProp}{65.7183}
\newcommand{\SevenSevenRProp}{65.6316}
\newcommand{\EightOneRProp}{71.0484}
\newcommand{\EightTenRProp}{73.4279}
\newcommand{\EightElevenRProp}{73.5029}
\newcommand{\EightTwelveRProp}{74.0291}
\newcommand{\EightThirteenRProp}{72.8291}
\newcommand{\EightFourteenRProp}{73.9226}
\newcommand{\EightFifteenRProp}{74.3344}
\newcommand{\EightSixteenRProp}{74.9213}
\newcommand{\EightSeventeenRProp}{74.5276}
\newcommand{\EightEighteenRProp}{74.9420}
\newcommand{\EightNineteenRProp}{61.0734}
\newcommand{\EightTwoOneRProp}{68.5198}
\newcommand{\EightTwoTenRProp}{73.6890}
\newcommand{\EightTwoElevenRProp}{73.0115}
\newcommand{\EightTwoTwelveRProp}{74.0194}
\newcommand{\EightTwoThirteenRProp}{74.1685}
\newcommand{\EightTwoFourteenRProp}{73.7000}
\newcommand{\EightTwoFifteenRProp}{64.3305}
\newcommand{\EightTwoSixteenRProp}{66.8434}
\newcommand{\EightTwoTwoRProp}{71.1823}
\newcommand{\EightTwoThreeRProp}{72.7498}
\newcommand{\EightTwoFourRProp}{72.6102}
\newcommand{\EightTwoFiveRProp}{74.0039}
\newcommand{\EightTwoSixRProp}{73.2932}
\newcommand{\EightTwoSevenRProp}{74.4165}
\newcommand{\EightTwoEightRProp}{73.7849}
\newcommand{\EightTwoNineRProp}{74.0620}
\newcommand{\EightTwoRProp}{71.4327}
\newcommand{\EightTwentyRProp}{63.1530}
\newcommand{\EightTwentyoneRProp}{65.5504}
\newcommand{\EightThreeOneRProp}{72.2883}
\newcommand{\EightThreeTenRProp}{68.9823}
\newcommand{\EightThreeTwoRProp}{72.9544}
\newcommand{\EightThreeThreeRProp}{74.9366}
\newcommand{\EightThreeFourRProp}{77.8544}
\newcommand{\EightThreeFiveRProp}{73.4286}
\newcommand{\EightThreeSixRProp}{74.7680}
\newcommand{\EightThreeSevenRProp}{60.6065}
\newcommand{\EightThreeEightRProp}{65.0637}
\newcommand{\EightThreeNineRProp}{70.1904}
\newcommand{\EightThreeRProp}{71.1880}
\newcommand{\EightFourOneRProp}{75.2901}
\newcommand{\EightFourTwoRProp}{67.4772}
\newcommand{\EightFourThreeRProp}{66.4140}
\newcommand{\EightFourRProp}{72.0301}
\newcommand{\EightFiveRProp}{72.2100}
\newcommand{\EightSixRProp}{72.5005}
\newcommand{\EightSevenRProp}{72.2447}
\newcommand{\EightEightRProp}{73.3533}
\newcommand{\EightNineRProp}{72.4717}
\newcommand{\NineOneRProp}{75.7507}
\newcommand{\NineTenRProp}{79.8161}
\newcommand{\NineElevenRProp}{80.3650}
\newcommand{\NineTwelveRProp}{80.1275}
\newcommand{\NineThirteenRProp}{80.6525}
\newcommand{\NineFourteenRProp}{80.1512}
\newcommand{\NineFifteenRProp}{82.1665}
\newcommand{\NineSixteenRProp}{80.1446}
\newcommand{\NineSeventeenRProp}{80.5792}
\newcommand{\NineEighteenRProp}{81.6230}
\newcommand{\NineNineteenRProp}{82.1828}
\newcommand{\NineTwoOneRProp}{78.7014}
\newcommand{\NineTwoTenRProp}{80.3964}
\newcommand{\NineTwoElevenRProp}{82.0513}
\newcommand{\NineTwoTwelveRProp}{81.9983}
\newcommand{\NineTwoThirteenRProp}{79.3586}
\newcommand{\NineTwoFourteenRProp}{80.7420}
\newcommand{\NineTwoFifteenRProp}{80.5805}
\newcommand{\NineTwoSixteenRProp}{81.4190}
\newcommand{\NineTwoSeventeenRProp}{81.2589}
\newcommand{\NineTwoEighteenRProp}{82.2739}
\newcommand{\NineTwoNineteenRProp}{79.4899}
\newcommand{\NineTwoTwoRProp}{79.5525}
\newcommand{\NineTwoTwentyRProp}{80.4176}
\newcommand{\NineTwoTwentyoneRProp}{81.2545}
\newcommand{\NineTwoTwentytwoRProp}{81.1318}
\newcommand{\NineTwoTwentythreeRProp}{80.4552}
\newcommand{\NineTwoTwentyfourRProp}{82.5780}
\newcommand{\NineTwoTwentyfiveRProp}{81.8205}
\newcommand{\NineTwoTwentysixRProp}{82.1200}
\newcommand{\NineTwoTwentysevenRProp}{81.3442}
\newcommand{\NineTwoTwentyeightRProp}{81.3869}
\newcommand{\NineTwoTwentynineRProp}{82.1780}
\newcommand{\NineTwoThreeRProp}{79.9725}
\newcommand{\NineTwoThirtyRProp}{82.2789}
\newcommand{\NineTwoThirtyoneRProp}{80.6125}
\newcommand{\NineTwoThirtytwoRProp}{81.4352}
\newcommand{\NineTwoThirtythreeRProp}{82.2167}
\newcommand{\NineTwoThirtyfourRProp}{81.8743}
\newcommand{\NineTwoThirtyfiveRProp}{81.3504}
\newcommand{\NineTwoThirtysixRProp}{80.7280}
\newcommand{\NineTwoThirtysevenRProp}{81.9353}
\newcommand{\NineTwoThirtyeightRProp}{82.7480}
\newcommand{\NineTwoThirtynineRProp}{81.9251}
\newcommand{\NineTwoFourRProp}{78.7248}
\newcommand{\NineTwoFortyRProp}{82.0090}
\newcommand{\NineTwoFortyoneRProp}{83.6167}
\newcommand{\NineTwoFortytwoRProp}{83.6493}
\newcommand{\NineTwoFortythreeRProp}{66.3264}
\newcommand{\NineTwoFortyfourRProp}{72.2518}
\newcommand{\NineTwoFortyfiveRProp}{71.3593}
\newcommand{\NineTwoFortysixRProp}{73.9646}
\newcommand{\NineTwoFortysevenRProp}{69.9602}
\newcommand{\NineTwoFortyeightRProp}{73.6781}
\newcommand{\NineTwoFortynineRProp}{66.0806}
\newcommand{\NineTwoFiveRProp}{79.6807}
\newcommand{\NineTwoFiftyRProp}{69.3690}
\newcommand{\NineTwoFiftyoneRProp}{70.5942}
\newcommand{\NineTwoFiftytwoRProp}{72.9916}
\newcommand{\NineTwoFiftythreeRProp}{68.0369}
\newcommand{\NineTwoFiftyfourRProp}{71.0385}
\newcommand{\NineTwoFiftyfiveRProp}{73.8423}
\newcommand{\NineTwoFiftysixRProp}{75.2439}
\newcommand{\NineTwoFiftysevenRProp}{73.8408}
\newcommand{\NineTwoFiftyeightRProp}{74.1911}
\newcommand{\NineTwoFiftynineRProp}{73.0481}
\newcommand{\NineTwoSixRProp}{81.1029}
\newcommand{\NineTwoSixtyRProp}{73.5734}
\newcommand{\NineTwoSixtyoneRProp}{69.3978}
\newcommand{\NineTwoSevenRProp}{81.1705}
\newcommand{\NineTwoEightRProp}{81.0999}
\newcommand{\NineTwoNineRProp}{80.3391}
\newcommand{\NineTwoRProp}{79.3059}
\newcommand{\NineTwentyRProp}{80.2543}
\newcommand{\NineTwentyoneRProp}{81.1336}
\newcommand{\NineTwentytwoRProp}{81.0714}
\newcommand{\NineTwentythreeRProp}{81.3164}
\newcommand{\NineTwentyfourRProp}{80.9933}
\newcommand{\NineTwentyfiveRProp}{81.1873}
\newcommand{\NineTwentysixRProp}{80.9352}
\newcommand{\NineTwentysevenRProp}{81.9473}
\newcommand{\NineTwentyeightRProp}{81.5694}
\newcommand{\NineTwentynineRProp}{81.8708}
\newcommand{\NineThreeOneRProp}{81.2897}
\newcommand{\NineThreeTenRProp}{82.3446}
\newcommand{\NineThreeElevenRProp}{82.0323}
\newcommand{\NineThreeTwelveRProp}{82.6345}
\newcommand{\NineThreeThirteenRProp}{72.2098}
\newcommand{\NineThreeFourteenRProp}{74.5697}
\newcommand{\NineThreeFifteenRProp}{74.3877}
\newcommand{\NineThreeSixteenRProp}{75.0664}
\newcommand{\NineThreeSeventeenRProp}{74.2972}
\newcommand{\NineThreeEighteenRProp}{72.5059}
\newcommand{\NineThreeNineteenRProp}{72.7143}
\newcommand{\NineThreeTwoRProp}{82.4507}
\newcommand{\NineThreeTwentyRProp}{76.3557}
\newcommand{\NineThreeTwentyoneRProp}{74.9369}
\newcommand{\NineThreeThreeRProp}{82.3127}
\newcommand{\NineThreeFourRProp}{82.5449}
\newcommand{\NineThreeFiveRProp}{80.7974}
\newcommand{\NineThreeSixRProp}{81.0235}
\newcommand{\NineThreeSevenRProp}{82.1986}
\newcommand{\NineThreeEightRProp}{81.1631}
\newcommand{\NineThreeNineRProp}{81.6200}
\newcommand{\NineThreeRProp}{78.5867}
\newcommand{\NineThirtyRProp}{81.8567}
\newcommand{\NineThirtyoneRProp}{81.7436}
\newcommand{\NineThirtytwoRProp}{81.5775}
\newcommand{\NineThirtythreeRProp}{82.8451}
\newcommand{\NineThirtyfourRProp}{82.3213}
\newcommand{\NineThirtyfiveRProp}{79.2495}
\newcommand{\NineThirtysixRProp}{81.0579}
\newcommand{\NineThirtysevenRProp}{81.5845}
\newcommand{\NineThirtyeightRProp}{81.8119}
\newcommand{\NineThirtynineRProp}{81.9490}
\newcommand{\NineFourOneRProp}{85.5620}
\newcommand{\NineFourRProp}{78.4117}
\newcommand{\NineFortyRProp}{81.7008}
\newcommand{\NineFortyoneRProp}{81.4929}
\newcommand{\NineFortytwoRProp}{69.6133}
\newcommand{\NineFortythreeRProp}{71.7062}
\newcommand{\NineFortyfourRProp}{71.6516}
\newcommand{\NineFortyfiveRProp}{74.9154}
\newcommand{\NineFortysixRProp}{68.6579}
\newcommand{\NineFortysevenRProp}{75.1289}
\newcommand{\NineFortyeightRProp}{74.2918}
\newcommand{\NineFortynineRProp}{74.0530}
\newcommand{\NineFiveRProp}{79.7877}
\newcommand{\NineSixRProp}{80.1326}
\newcommand{\NineSevenRProp}{80.6597}
\newcommand{\NineEightRProp}{80.5651}
\newcommand{\NineNineRProp}{79.9574}


==> latex_knot_rub.tex <==
\newcommand{\TwoTwoOneRRUB}{25.1388}
\newcommand{\ThreeOneRRUB}{32.7448}
\newcommand{\FourOneRRUB}{42.0928}
\newcommand{\FourTwoOneRRUB}{40.0169}
\newcommand{\FiveOneRRUB}{47.2016}
\newcommand{\FiveTwoOneRRUB}{49.7723}
\newcommand{\FiveTwoRRUB}{49.4704}
\newcommand{\SixOneRRUB}{56.7150}
\newcommand{\SixTwoOneRRUB}{54.3893}
\newcommand{\SixTwoTwoRRUB}{56.7028}
\newcommand{\SixTwoThreeRRUB}{58.1044}
\newcommand{\SixTwoRRUB}{57.0271}
\newcommand{\SixThreeOneRRUB}{57.8170}
\newcommand{\SixThreeTwoRRUB}{58.0145}
\newcommand{\SixThreeThreeRRUB}{50.5745}
\newcommand{\SixThreeRRUB}{57.8435}
\newcommand{\SevenOneRRUB}{61.4109}
\newcommand{\SevenTwoOneRRUB}{64.2353}
\newcommand{\SevenTwoTwoRRUB}{65.0274}
\newcommand{\SevenTwoThreeRRUB}{65.3561}
\newcommand{\SevenTwoFourRRUB}{65.0759}
\newcommand{\SevenTwoFiveRRUB}{66.2186}
\newcommand{\SevenTwoSixRRUB}{66.3372}
\newcommand{\SevenTwoSevenRRUB}{55.5311}
\newcommand{\SevenTwoEightRRUB}{57.7948}
\newcommand{\SevenTwoRRUB}{63.8956}
\newcommand{\SevenThreeOneRRUB}{65.8090}
\newcommand{\SevenThreeRRUB}{63.9327}
\newcommand{\SevenFourRRUB}{64.2724}
\newcommand{\SevenFiveRRUB}{65.2609}
\newcommand{\SevenSixRRUB}{65.7012}
\newcommand{\SevenSevenRRUB}{65.6108}
\newcommand{\EightOneRRUB}{71.0241}
\newcommand{\EightTenRRUB}{73.4095}
\newcommand{\EightElevenRRUB}{73.4802}
\newcommand{\EightTwelveRRUB}{74.0098}
\newcommand{\EightThirteenRRUB}{72.8045}
\newcommand{\EightFourteenRRUB}{73.8991}
\newcommand{\EightFifteenRRUB}{74.3134}
\newcommand{\EightSixteenRRUB}{74.8962}
\newcommand{\EightSeventeenRRUB}{74.5071}
\newcommand{\EightEighteenRRUB}{74.9252}
\newcommand{\EightNineteenRRUB}{61.0430}
\newcommand{\EightTwoOneRRUB}{68.4884}
\newcommand{\EightTwoTenRRUB}{73.6684}
\newcommand{\EightTwoElevenRRUB}{72.9899}
\newcommand{\EightTwoTwelveRRUB}{73.9140}
\newcommand{\EightTwoThirteenRRUB}{74.1501}
\newcommand{\EightTwoFourteenRRUB}{73.6775}
\newcommand{\EightTwoFifteenRRUB}{64.3086}
\newcommand{\EightTwoSixteenRRUB}{66.8315}
\newcommand{\EightTwoTwoRRUB}{71.1587}
\newcommand{\EightTwoThreeRRUB}{72.7291}
\newcommand{\EightTwoFourRRUB}{72.5908}
\newcommand{\EightTwoFiveRRUB}{73.9826}
\newcommand{\EightTwoSixRRUB}{73.2502}
\newcommand{\EightTwoSevenRRUB}{74.3885}
\newcommand{\EightTwoEightRRUB}{73.7702}
\newcommand{\EightTwoNineRRUB}{74.0386}
\newcommand{\EightTwoRRUB}{71.4107}
\newcommand{\EightTwentyRRUB}{63.1146}
\newcommand{\EightTwentyoneRRUB}{65.5298}
\newcommand{\EightThreeOneRRUB}{72.2649}
\newcommand{\EightThreeTenRRUB}{68.9694}
\newcommand{\EightThreeTwoRRUB}{72.9360}
\newcommand{\EightThreeThreeRRUB}{74.9139}
\newcommand{\EightThreeFourRRUB}{77.8314}
\newcommand{\EightThreeFiveRRUB}{73.4061}
\newcommand{\EightThreeSixRRUB}{74.7468}
\newcommand{\EightThreeSevenRRUB}{60.5888}
\newcommand{\EightThreeEightRRUB}{65.0444}
\newcommand{\EightThreeNineRRUB}{70.1810}
\newcommand{\EightThreeRRUB}{71.1655}
\newcommand{\EightFourOneRRUB}{75.2677}
\newcommand{\EightFourTwoRRUB}{67.4571}
\newcommand{\EightFourThreeRRUB}{66.4046}
\newcommand{\EightFourRRUB}{72.0049}
\newcommand{\EightFiveRRUB}{72.1878}
\newcommand{\EightSixRRUB}{72.4791}
\newcommand{\EightSevenRRUB}{72.2204}
\newcommand{\EightEightRRUB}{73.3334}
\newcommand{\EightNineRRUB}{72.4461}
\newcommand{\NineOneRRUB}{75.7252}
\newcommand{\NineTenRRUB}{79.7946}
\newcommand{\NineElevenRRUB}{80.3418}
\newcommand{\NineTwelveRRUB}{80.1047}
\newcommand{\NineThirteenRRUB}{80.6246}
\newcommand{\NineFourteenRRUB}{80.1259}
\newcommand{\NineFifteenRRUB}{82.1396}
\newcommand{\NineSixteenRRUB}{80.1211}
\newcommand{\NineSeventeenRRUB}{80.5537}
\newcommand{\NineEighteenRRUB}{81.5960}
\newcommand{\NineNineteenRRUB}{82.1593}
\newcommand{\NineTwoOneRRUB}{78.6731}
\newcommand{\NineTwoTenRRUB}{80.3693}
\newcommand{\NineTwoElevenRRUB}{82.0271}
\newcommand{\NineTwoTwelveRRUB}{81.9738}
\newcommand{\NineTwoThirteenRRUB}{79.3319}
\newcommand{\NineTwoFourteenRRUB}{80.7171}
\newcommand{\NineTwoFifteenRRUB}{80.5550}
\newcommand{\NineTwoSixteenRRUB}{81.3966}
\newcommand{\NineTwoSeventeenRRUB}{81.2307}
\newcommand{\NineTwoEighteenRRUB}{82.2429}
\newcommand{\NineTwoNineteenRRUB}{79.4628}
\newcommand{\NineTwoTwoRRUB}{79.5259}
\newcommand{\NineTwoTwentyRRUB}{80.3956}
\newcommand{\NineTwoTwentyoneRRUB}{81.2356}
\newcommand{\NineTwoTwentytwoRRUB}{81.1058}
\newcommand{\NineTwoTwentythreeRRUB}{80.4290}
\newcommand{\NineTwoTwentyfourRRUB}{82.5207}
\newcommand{\NineTwoTwentyfiveRRUB}{81.7924}
\newcommand{\NineTwoTwentysixRRUB}{82.1015}
\newcommand{\NineTwoTwentysevenRRUB}{81.2046}
\newcommand{\NineTwoTwentyeightRRUB}{81.3740}
\newcommand{\NineTwoTwentynineRRUB}{82.1567}
\newcommand{\NineTwoThreeRRUB}{79.9476}
\newcommand{\NineTwoThirtyRRUB}{82.2517}
\newcommand{\NineTwoThirtyoneRRUB}{80.5936}
\newcommand{\NineTwoThirtytwoRRUB}{81.4122}
\newcommand{\NineTwoThirtythreeRRUB}{82.1951}
\newcommand{\NineTwoThirtyfourRRUB}{81.8552}
\newcommand{\NineTwoThirtyfiveRRUB}{81.3284}
\newcommand{\NineTwoThirtysixRRUB}{80.7103}
\newcommand{\NineTwoThirtysevenRRUB}{81.9101}
\newcommand{\NineTwoThirtyeightRRUB}{82.7206}
\newcommand{\NineTwoThirtynineRRUB}{81.8973}
\newcommand{\NineTwoFourRRUB}{78.6967}
\newcommand{\NineTwoFortyRRUB}{81.9822}
\newcommand{\NineTwoFortyoneRRUB}{83.5979}
\newcommand{\NineTwoFortytwoRRUB}{83.6292}
\newcommand{\NineTwoFortythreeRRUB}{66.3049}
\newcommand{\NineTwoFortyfourRRUB}{72.2255}
\newcommand{\NineTwoFortyfiveRRUB}{71.3490}
\newcommand{\NineTwoFortysixRRUB}{73.9377}
\newcommand{\NineTwoFortysevenRRUB}{69.9432}
\newcommand{\NineTwoFortyeightRRUB}{73.6545}
\newcommand{\NineTwoFortynineRRUB}{66.0658}
\newcommand{\NineTwoFiveRRUB}{79.6549}
\newcommand{\NineTwoFiftyRRUB}{69.3483}
\newcommand{\NineTwoFiftyoneRRUB}{70.5699}
\newcommand{\NineTwoFiftytwoRRUB}{72.9685}
\newcommand{\NineTwoFiftythreeRRUB}{68.0305}
\newcommand{\NineTwoFiftyfourRRUB}{71.0185}
\newcommand{\NineTwoFiftyfiveRRUB}{73.8217}
\newcommand{\NineTwoFiftysixRRUB}{75.2245}
\newcommand{\NineTwoFiftysevenRRUB}{73.8194}
\newcommand{\NineTwoFiftyeightRRUB}{74.1697}
\newcommand{\NineTwoFiftynineRRUB}{73.0305}
\newcommand{\NineTwoSixRRUB}{81.0791}
\newcommand{\NineTwoSixtyRRUB}{73.5553}
\newcommand{\NineTwoSixtyoneRRUB}{69.3840}
\newcommand{\NineTwoSevenRRUB}{81.1460}
\newcommand{\NineTwoEightRRUB}{81.0723}
\newcommand{\NineTwoNineRRUB}{80.3181}
\newcommand{\NineTwoRRUB}{79.2794}
\newcommand{\NineTwentyRRUB}{80.2288}
\newcommand{\NineTwentyoneRRUB}{81.1098}
\newcommand{\NineTwentytwoRRUB}{81.0464}
\newcommand{\NineTwentythreeRRUB}{81.2898}
\newcommand{\NineTwentyfourRRUB}{80.9701}
\newcommand{\NineTwentyfiveRRUB}{81.1612}
\newcommand{\NineTwentysixRRUB}{80.9137}
\newcommand{\NineTwentysevenRRUB}{81.9092}
\newcommand{\NineTwentyeightRRUB}{81.5467}
\newcommand{\NineTwentynineRRUB}{81.8470}
\newcommand{\NineThreeOneRRUB}{81.2323}
\newcommand{\NineThreeTenRRUB}{82.3259}
\newcommand{\NineThreeElevenRRUB}{82.0137}
\newcommand{\NineThreeTwelveRRUB}{82.5740}
\newcommand{\NineThreeThirteenRRUB}{72.2008}
\newcommand{\NineThreeFourteenRRUB}{74.5492}
\newcommand{\NineThreeFifteenRRUB}{74.3655}
\newcommand{\NineThreeSixteenRRUB}{75.0430}
\newcommand{\NineThreeSeventeenRRUB}{74.2779}
\newcommand{\NineThreeEighteenRRUB}{72.4741}
\newcommand{\NineThreeNineteenRRUB}{72.6859}
\newcommand{\NineThreeTwoRRUB}{82.4004}
\newcommand{\NineThreeTwentyRRUB}{76.1829}
\newcommand{\NineThreeTwentyoneRRUB}{74.9212}
\newcommand{\NineThreeThreeRRUB}{82.2861}
\newcommand{\NineThreeFourRRUB}{82.5208}
\newcommand{\NineThreeFiveRRUB}{80.7714}
\newcommand{\NineThreeSixRRUB}{81.0054}
\newcommand{\NineThreeSevenRRUB}{82.1535}
\newcommand{\NineThreeEightRRUB}{81.1408}
\newcommand{\NineThreeNineRRUB}{81.5735}
\newcommand{\NineThreeRRUB}{78.5591}
\newcommand{\NineThirtyRRUB}{81.8344}
\newcommand{\NineThirtyoneRRUB}{81.6915}
\newcommand{\NineThirtytwoRRUB}{81.5555}
\newcommand{\NineThirtythreeRRUB}{82.7989}
\newcommand{\NineThirtyfourRRUB}{82.2744}
\newcommand{\NineThirtyfiveRRUB}{79.2216}
\newcommand{\NineThirtysixRRUB}{81.0297}
\newcommand{\NineThirtysevenRRUB}{81.5562}
\newcommand{\NineThirtyeightRRUB}{81.7909}
\newcommand{\NineThirtynineRRUB}{81.9266}
\newcommand{\NineFourOneRRUB}{85.5115}
\newcommand{\NineFourRRUB}{78.3861}
\newcommand{\NineFortyRRUB}{81.6806}
\newcommand{\NineFortyoneRRUB}{81.4399}
\newcommand{\NineFortytwoRRUB}{69.5939}
\newcommand{\NineFortythreeRRUB}{71.6863}
\newcommand{\NineFortyfourRRUB}{71.6305}
\newcommand{\NineFortyfiveRRUB}{74.8959}
\newcommand{\NineFortysixRRUB}{68.6369}
\newcommand{\NineFortysevenRRUB}{75.0875}
\newcommand{\NineFortyeightRRUB}{74.2477}
\newcommand{\NineFortynineRRUB}{74.0127}
\newcommand{\NineFiveRRUB}{79.7586}
\newcommand{\NineSixRRUB}{80.0822}
\newcommand{\NineSevenRRUB}{80.6357}
\newcommand{\NineEightRRUB}{80.5384}
\newcommand{\NineNineRRUB}{79.9323}


==> latex_knot_vert.tex <==
\newcommand{\TwoTwoOneVert}{179}
\newcommand{\TwoTwoOneSym}{2^{2}_{1}}
\newcommand{\ThreeOneVert}{400}
\newcommand{\ThreeOneSym}{3_{1}}
\newcommand{\FourOneVert}{400}
\newcommand{\FourOneSym}{4_{1}}
\newcommand{\FourTwoOneVert}{400}
\newcommand{\FourTwoOneSym}{4^{2}_{1}}
\newcommand{\FiveOneVert}{400}
\newcommand{\FiveOneSym}{5_{1}}
\newcommand{\FiveTwoOneVert}{400}
\newcommand{\FiveTwoOneSym}{5^{2}_{1}}
\newcommand{\FiveTwoVert}{400}
\newcommand{\FiveTwoSym}{5_{2}}
\newcommand{\SixOneVert}{405}
\newcommand{\SixOneSym}{6_{1}}
\newcommand{\SixTwoOneVert}{400}
\newcommand{\SixTwoOneSym}{6^{2}_{1}}
\newcommand{\SixTwoTwoVert}{562}
\newcommand{\SixTwoTwoSym}{6^{2}_{2}}
\newcommand{\SixTwoThreeVert}{558}
\newcommand{\SixTwoThreeSym}{6^{2}_{3}}
\newcommand{\SixTwoVert}{407}
\newcommand{\SixTwoSym}{6_{2}}
\newcommand{\SixThreeOneVert}{413}
\newcommand{\SixThreeOneSym}{6^{3}_{1}}
\newcommand{\SixThreeTwoVert}{451}
\newcommand{\SixThreeTwoSym}{6^{3}_{2}}
\newcommand{\SixThreeThreeVert}{362}
\newcommand{\SixThreeThreeSym}{6^{3}_{3}}
\newcommand{\SixThreeVert}{413}
\newcommand{\SixThreeSym}{6_{3}}
\newcommand{\SevenOneVert}{438}
\newcommand{\SevenOneSym}{7_{1}}
\newcommand{\SevenTwoOneVert}{459}
\newcommand{\SevenTwoOneSym}{7^{2}_{1}}
\newcommand{\SevenTwoTwoVert}{464}
\newcommand{\SevenTwoTwoSym}{7^{2}_{2}}
\newcommand{\SevenTwoThreeVert}{467}
\newcommand{\SevenTwoThreeSym}{7^{2}_{3}}
\newcommand{\SevenTwoFourVert}{465}
\newcommand{\SevenTwoFourSym}{7^{2}_{4}}
\newcommand{\SevenTwoFiveVert}{473}
\newcommand{\SevenTwoFiveSym}{7^{2}_{5}}
\newcommand{\SevenTwoSixVert}{474}
\newcommand{\SevenTwoSixSym}{7^{2}_{6}}
\newcommand{\SevenTwoSevenVert}{400}
\newcommand{\SevenTwoSevenSym}{7^{2}_{7}}
\newcommand{\SevenTwoEightVert}{619}
\newcommand{\SevenTwoEightSym}{7^{2}_{8}}
\newcommand{\SevenTwoVert}{456}
\newcommand{\SevenTwoSym}{7_{2}}
\newcommand{\SevenThreeOneVert}{470}
\newcommand{\SevenThreeOneSym}{7^{3}_{1}}
\newcommand{\SevenThreeVert}{456}
\newcommand{\SevenThreeSym}{7_{3}}
\newcommand{\SevenFourVert}{459}
\newcommand{\SevenFourSym}{7_{4}}
\newcommand{\SevenFiveVert}{466}
\newcommand{\SevenFiveSym}{7_{5}}
\newcommand{\SevenSixVert}{469}
\newcommand{\SevenSixSym}{7_{6}}
\newcommand{\SevenSevenVert}{468}
\newcommand{\SevenSevenSym}{7_{7}}
\newcommand{\EightOneVert}{507}
\newcommand{\EightOneSym}{8_{1}}
\newcommand{\EightTenVert}{524}
\newcommand{\EightTenSym}{8_{10}}
\newcommand{\EightElevenVert}{525}
\newcommand{\EightElevenSym}{8_{11}}
\newcommand{\EightTwelveVert}{529}
\newcommand{\EightTwelveSym}{8_{12}}
\newcommand{\EightThirteenVert}{520}
\newcommand{\EightThirteenSym}{8_{13}}
\newcommand{\EightFourteenVert}{528}
\newcommand{\EightFourteenSym}{8_{14}}
\newcommand{\EightFifteenVert}{531}
\newcommand{\EightFifteenSym}{8_{15}}
\newcommand{\EightSixteenVert}{535}
\newcommand{\EightSixteenSym}{8_{16}}
\newcommand{\EightSeventeenVert}{532}
\newcommand{\EightSeventeenSym}{8_{17}}
\newcommand{\EightEighteenVert}{535}
\newcommand{\EightEighteenSym}{8_{18}}
\newcommand{\EightNineteenVert}{304}
\newcommand{\EightNineteenSym}{8_{19}}
\newcommand{\EightTwoOneVert}{489}
\newcommand{\EightTwoOneSym}{8^{2}_{1}}
\newcommand{\EightTwoTenVert}{526}
\newcommand{\EightTwoTenSym}{8^{2}_{10}}
\newcommand{\EightTwoElevenVert}{521}
\newcommand{\EightTwoElevenSym}{8^{2}_{11}}
\newcommand{\EightTwoTwelveVert}{200}
\newcommand{\EightTwoTwelveSym}{8^{2}_{12}}
\newcommand{\EightTwoThirteenVert}{529}
\newcommand{\EightTwoThirteenSym}{8^{2}_{13}}
\newcommand{\EightTwoFourteenVert}{526}
\newcommand{\EightTwoFourteenSym}{8^{2}_{14}}
\newcommand{\EightTwoFifteenVert}{459}
\newcommand{\EightTwoFifteenSym}{8^{2}_{15}}
\newcommand{\EightTwoSixteenVert}{477}
\newcommand{\EightTwoSixteenSym}{8^{2}_{16}}
\newcommand{\EightTwoTwoVert}{508}
\newcommand{\EightTwoTwoSym}{8^{2}_{2}}
\newcommand{\EightTwoThreeVert}{519}
\newcommand{\EightTwoThreeSym}{8^{2}_{3}}
\newcommand{\EightTwoFourVert}{518}
\newcommand{\EightTwoFourSym}{8^{2}_{4}}
\newcommand{\EightTwoFiveVert}{528}
\newcommand{\EightTwoFiveSym}{8^{2}_{5}}
\newcommand{\EightTwoSixVert}{447}
\newcommand{\EightTwoSixSym}{8^{2}_{6}}
\newcommand{\EightTwoSevenVert}{531}
\newcommand{\EightTwoSevenSym}{8^{2}_{7}}
\newcommand{\EightTwoEightVert}{527}
\newcommand{\EightTwoEightSym}{8^{2}_{8}}
\newcommand{\EightTwoNineVert}{529}
\newcommand{\EightTwoNineSym}{8^{2}_{9}}
\newcommand{\EightTwoVert}{510}
\newcommand{\EightTwoSym}{8_{2}}
\newcommand{\EightTwentyVert}{312}
\newcommand{\EightTwentySym}{8_{20}}
\newcommand{\EightTwentyoneVert}{468}
\newcommand{\EightTwentyoneSym}{8_{21}}
\newcommand{\EightThreeOneVert}{517}
\newcommand{\EightThreeOneSym}{8^{3}_{1}}
\newcommand{\EightThreeTenVert}{507}
\newcommand{\EightThreeTenSym}{8^{3}_{10}}
\newcommand{\EightThreeTwoVert}{521}
\newcommand{\EightThreeTwoSym}{8^{3}_{2}}
\newcommand{\EightThreeThreeVert}{535}
\newcommand{\EightThreeThreeSym}{8^{3}_{3}}
\newcommand{\EightThreeFourVert}{556}
\newcommand{\EightThreeFourSym}{8^{3}_{4}}
\newcommand{\EightThreeFiveVert}{524}
\newcommand{\EightThreeFiveSym}{8^{3}_{5}}
\newcommand{\EightThreeSixVert}{534}
\newcommand{\EightThreeSixSym}{8^{3}_{6}}
\newcommand{\EightThreeSevenVert}{432}
\newcommand{\EightThreeSevenSym}{8^{3}_{7}}
\newcommand{\EightThreeEightVert}{464}
\newcommand{\EightThreeEightSym}{8^{3}_{8}}
\newcommand{\EightThreeNineVert}{651}
\newcommand{\EightThreeNineSym}{8^{3}_{9}}
\newcommand{\EightThreeVert}{508}
\newcommand{\EightThreeSym}{8_{3}}
\newcommand{\EightFourOneVert}{536}
\newcommand{\EightFourOneSym}{8^{4}_{1}}
\newcommand{\EightFourTwoVert}{482}
\newcommand{\EightFourTwoSym}{8^{4}_{2}}
\newcommand{\EightFourThreeVert}{476}
\newcommand{\EightFourThreeSym}{8^{4}_{3}}
\newcommand{\EightFourVert}{514}
\newcommand{\EightFourSym}{8_{4}}
\newcommand{\EightFiveVert}{516}
\newcommand{\EightFiveSym}{8_{5}}
\newcommand{\EightSixVert}{518}
\newcommand{\EightSixSym}{8_{6}}
\newcommand{\EightSevenVert}{516}
\newcommand{\EightSevenSym}{8_{7}}
\newcommand{\EightEightVert}{523}
\newcommand{\EightEightSym}{8_{8}}
\newcommand{\EightNineVert}{517}
\newcommand{\EightNineSym}{8_{9}}
\newcommand{\NineOneVert}{541}
\newcommand{\NineOneSym}{9_{1}}
\newcommand{\NineTenVert}{570}
\newcommand{\NineTenSym}{9_{10}}
\newcommand{\NineElevenVert}{574}
\newcommand{\NineElevenSym}{9_{11}}
\newcommand{\NineTwelveVert}{572}
\newcommand{\NineTwelveSym}{9_{12}}
\newcommand{\NineThirteenVert}{576}
\newcommand{\NineThirteenSym}{9_{13}}
\newcommand{\NineFourteenVert}{572}
\newcommand{\NineFourteenSym}{9_{14}}
\newcommand{\NineFifteenVert}{587}
\newcommand{\NineFifteenSym}{9_{15}}
\newcommand{\NineSixteenVert}{572}
\newcommand{\NineSixteenSym}{9_{16}}
\newcommand{\NineSeventeenVert}{575}
\newcommand{\NineSeventeenSym}{9_{17}}
\newcommand{\NineEighteenVert}{583}
\newcommand{\NineEighteenSym}{9_{18}}
\newcommand{\NineNineteenVert}{587}
\newcommand{\NineNineteenSym}{9_{19}}
\newcommand{\NineTwoOneVert}{562}
\newcommand{\NineTwoOneSym}{9^{2}_{1}}
\newcommand{\NineTwoTenVert}{574}
\newcommand{\NineTwoTenSym}{9^{2}_{10}}
\newcommand{\NineTwoElevenVert}{586}
\newcommand{\NineTwoElevenSym}{9^{2}_{11}}
\newcommand{\NineTwoTwelveVert}{586}
\newcommand{\NineTwoTwelveSym}{9^{2}_{12}}
\newcommand{\NineTwoThirteenVert}{567}
\newcommand{\NineTwoThirteenSym}{9^{2}_{13}}
\newcommand{\NineTwoFourteenVert}{577}
\newcommand{\NineTwoFourteenSym}{9^{2}_{14}}
\newcommand{\NineTwoFifteenVert}{575}
\newcommand{\NineTwoFifteenSym}{9^{2}_{15}}
\newcommand{\NineTwoSixteenVert}{581}
\newcommand{\NineTwoSixteenSym}{9^{2}_{16}}
\newcommand{\NineTwoSeventeenVert}{580}
\newcommand{\NineTwoSeventeenSym}{9^{2}_{17}}
\newcommand{\NineTwoEighteenVert}{588}
\newcommand{\NineTwoEighteenSym}{9^{2}_{18}}
\newcommand{\NineTwoNineteenVert}{568}
\newcommand{\NineTwoNineteenSym}{9^{2}_{19}}
\newcommand{\NineTwoTwoVert}{568}
\newcommand{\NineTwoTwoSym}{9^{2}_{2}}
\newcommand{\NineTwoTwentyVert}{575}
\newcommand{\NineTwoTwentySym}{9^{2}_{20}}
\newcommand{\NineTwoTwentyoneVert}{613}
\newcommand{\NineTwoTwentyoneSym}{9^{2}_{21}}
\newcommand{\NineTwoTwentytwoVert}{579}
\newcommand{\NineTwoTwentytwoSym}{9^{2}_{22}}
\newcommand{\NineTwoTwentythreeVert}{574}
\newcommand{\NineTwoTwentythreeSym}{9^{2}_{23}}
\newcommand{\NineTwoTwentyfourVert}{400}
\newcommand{\NineTwoTwentyfourSym}{9^{2}_{24}}
\newcommand{\NineTwoTwentyfiveVert}{584}
\newcommand{\NineTwoTwentyfiveSym}{9^{2}_{25}}
\newcommand{\NineTwoTwentysixVert}{586}
\newcommand{\NineTwoTwentysixSym}{9^{2}_{26}}
\newcommand{\NineTwoTwentysevenVert}{200}
\newcommand{\NineTwoTwentysevenSym}{9^{2}_{27}}
\newcommand{\NineTwoTwentyeightVert}{581}
\newcommand{\NineTwoTwentyeightSym}{9^{2}_{28}}
\newcommand{\NineTwoTwentynineVert}{588}
\newcommand{\NineTwoTwentynineSym}{9^{2}_{29}}
\newcommand{\NineTwoThreeVert}{571}
\newcommand{\NineTwoThreeSym}{9^{2}_{3}}
\newcommand{\NineTwoThirtyVert}{588}
\newcommand{\NineTwoThirtySym}{9^{2}_{30}}
\newcommand{\NineTwoThirtyoneVert}{576}
\newcommand{\NineTwoThirtyoneSym}{9^{2}_{31}}
\newcommand{\NineTwoThirtytwoVert}{581}
\newcommand{\NineTwoThirtytwoSym}{9^{2}_{32}}
\newcommand{\NineTwoThirtythreeVert}{587}
\newcommand{\NineTwoThirtythreeSym}{9^{2}_{33}}
\newcommand{\NineTwoThirtyfourVert}{585}
\newcommand{\NineTwoThirtyfourSym}{9^{2}_{34}}
\newcommand{\NineTwoThirtyfiveVert}{580}
\newcommand{\NineTwoThirtyfiveSym}{9^{2}_{35}}
\newcommand{\NineTwoThirtysixVert}{576}
\newcommand{\NineTwoThirtysixSym}{9^{2}_{36}}
\newcommand{\NineTwoThirtysevenVert}{585}
\newcommand{\NineTwoThirtysevenSym}{9^{2}_{37}}
\newcommand{\NineTwoThirtyeightVert}{591}
\newcommand{\NineTwoThirtyeightSym}{9^{2}_{38}}
\newcommand{\NineTwoThirtynineVert}{585}
\newcommand{\NineTwoThirtynineSym}{9^{2}_{39}}
\newcommand{\NineTwoFourVert}{562}
\newcommand{\NineTwoFourSym}{9^{2}_{4}}
\newcommand{\NineTwoFortyVert}{586}
\newcommand{\NineTwoFortySym}{9^{2}_{40}}
\newcommand{\NineTwoFortyoneVert}{597}
\newcommand{\NineTwoFortyoneSym}{9^{2}_{41}}
\newcommand{\NineTwoFortytwoVert}{597}
\newcommand{\NineTwoFortytwoSym}{9^{2}_{42}}
\newcommand{\NineTwoFortythreeVert}{473}
\newcommand{\NineTwoFortythreeSym}{9^{2}_{43}}
\newcommand{\NineTwoFortyfourVert}{516}
\newcommand{\NineTwoFortyfourSym}{9^{2}_{44}}
\newcommand{\NineTwoFortyfiveVert}{886}
\newcommand{\NineTwoFortyfiveSym}{9^{2}_{45}}
\newcommand{\NineTwoFortysixVert}{528}
\newcommand{\NineTwoFortysixSym}{9^{2}_{46}}
\newcommand{\NineTwoFortysevenVert}{657}
\newcommand{\NineTwoFortysevenSym}{9^{2}_{47}}
\newcommand{\NineTwoFortyeightVert}{564}
\newcommand{\NineTwoFortyeightSym}{9^{2}_{48}}
\newcommand{\NineTwoFortynineVert}{472}
\newcommand{\NineTwoFortynineSym}{9^{2}_{49}}
\newcommand{\NineTwoFiveVert}{569}
\newcommand{\NineTwoFiveSym}{9^{2}_{5}}
\newcommand{\NineTwoFiftyVert}{495}
\newcommand{\NineTwoFiftySym}{9^{2}_{50}}
\newcommand{\NineTwoFiftyoneVert}{504}
\newcommand{\NineTwoFiftyoneSym}{9^{2}_{51}}
\newcommand{\NineTwoFiftytwoVert}{522}
\newcommand{\NineTwoFiftytwoSym}{9^{2}_{52}}
\newcommand{\NineTwoFiftythreeVert}{755}
\newcommand{\NineTwoFiftythreeSym}{9^{2}_{53}}
\newcommand{\NineTwoFiftyfourVert}{507}
\newcommand{\NineTwoFiftyfourSym}{9^{2}_{54}}
\newcommand{\NineTwoFiftyfiveVert}{527}
\newcommand{\NineTwoFiftyfiveSym}{9^{2}_{55}}
\newcommand{\NineTwoFiftysixVert}{537}
\newcommand{\NineTwoFiftysixSym}{9^{2}_{56}}
\newcommand{\NineTwoFiftysevenVert}{527}
\newcommand{\NineTwoFiftysevenSym}{9^{2}_{57}}
\newcommand{\NineTwoFiftyeightVert}{530}
\newcommand{\NineTwoFiftyeightSym}{9^{2}_{58}}
\newcommand{\NineTwoFiftynineVert}{522}
\newcommand{\NineTwoFiftynineSym}{9^{2}_{59}}
\newcommand{\NineTwoSixVert}{579}
\newcommand{\NineTwoSixSym}{9^{2}_{6}}
\newcommand{\NineTwoSixtyVert}{526}
\newcommand{\NineTwoSixtySym}{9^{2}_{60}}
\newcommand{\NineTwoSixtyoneVert}{495}
\newcommand{\NineTwoSixtyoneSym}{9^{2}_{61}}
\newcommand{\NineTwoSevenVert}{580}
\newcommand{\NineTwoSevenSym}{9^{2}_{7}}
\newcommand{\NineTwoEightVert}{579}
\newcommand{\NineTwoEightSym}{9^{2}_{8}}
\newcommand{\NineTwoNineVert}{575}
\newcommand{\NineTwoNineSym}{9^{2}_{9}}
\newcommand{\NineTwoVert}{566}
\newcommand{\NineTwoSym}{9_{2}}
\newcommand{\NineTwentyVert}{573}
\newcommand{\NineTwentySym}{9_{20}}
\newcommand{\NineTwentyoneVert}{579}
\newcommand{\NineTwentyoneSym}{9_{21}}
\newcommand{\NineTwentytwoVert}{579}
\newcommand{\NineTwentytwoSym}{9_{22}}
\newcommand{\NineTwentythreeVert}{581}
\newcommand{\NineTwentythreeSym}{9_{23}}
\newcommand{\NineTwentyfourVert}{578}
\newcommand{\NineTwentyfourSym}{9_{24}}
\newcommand{\NineTwentyfiveVert}{580}
\newcommand{\NineTwentyfiveSym}{9_{25}}
\newcommand{\NineTwentysixVert}{578}
\newcommand{\NineTwentysixSym}{9_{26}}
\newcommand{\NineTwentysevenVert}{408}
\newcommand{\NineTwentysevenSym}{9_{27}}
\newcommand{\NineTwentyeightVert}{582}
\newcommand{\NineTwentyeightSym}{9_{28}}
\newcommand{\NineTwentynineVert}{585}
\newcommand{\NineTwentynineSym}{9_{29}}
\newcommand{\NineThreeOneVert}{400}
\newcommand{\NineThreeOneSym}{9^{3}_{1}}
\newcommand{\NineThreeTenVert}{588}
\newcommand{\NineThreeTenSym}{9^{3}_{10}}
\newcommand{\NineThreeElevenVert}{584}
\newcommand{\NineThreeElevenSym}{9^{3}_{11}}
\newcommand{\NineThreeTwelveVert}{400}
\newcommand{\NineThreeTwelveSym}{9^{3}_{12}}
\newcommand{\NineThreeThirteenVert}{875}
\newcommand{\NineThreeThirteenSym}{9^{3}_{13}}
\newcommand{\NineThreeFourteenVert}{532}
\newcommand{\NineThreeFourteenSym}{9^{3}_{14}}
\newcommand{\NineThreeFifteenVert}{530}
\newcommand{\NineThreeFifteenSym}{9^{3}_{15}}
\newcommand{\NineThreeSixteenVert}{535}
\newcommand{\NineThreeSixteenSym}{9^{3}_{16}}
\newcommand{\NineThreeSeventeenVert}{529}
\newcommand{\NineThreeSeventeenSym}{9^{3}_{17}}
\newcommand{\NineThreeEighteenVert}{400}
\newcommand{\NineThreeEighteenSym}{9^{3}_{18}}
\newcommand{\NineThreeNineteenVert}{400}
\newcommand{\NineThreeNineteenSym}{9^{3}_{19}}
\newcommand{\NineThreeTwoVert}{400}
\newcommand{\NineThreeTwoSym}{9^{3}_{2}}
\newcommand{\NineThreeTwentyVert}{200}
\newcommand{\NineThreeTwentySym}{9^{3}_{20}}
\newcommand{\NineThreeTwentyoneVert}{566}
\newcommand{\NineThreeTwentyoneSym}{9^{3}_{21}}
\newcommand{\NineThreeThreeVert}{589}
\newcommand{\NineThreeThreeSym}{9^{3}_{3}}
\newcommand{\NineThreeFourVert}{591}
\newcommand{\NineThreeFourSym}{9^{3}_{4}}
\newcommand{\NineThreeFiveVert}{575}
\newcommand{\NineThreeFiveSym}{9^{3}_{5}}
\newcommand{\NineThreeSixVert}{586}
\newcommand{\NineThreeSixSym}{9^{3}_{6}}
\newcommand{\NineThreeSevenVert}{400}
\newcommand{\NineThreeSevenSym}{9^{3}_{7}}
\newcommand{\NineThreeEightVert}{585}
\newcommand{\NineThreeEightSym}{9^{3}_{8}}
\newcommand{\NineThreeNineVert}{400}
\newcommand{\NineThreeNineSym}{9^{3}_{9}}
\newcommand{\NineThreeVert}{561}
\newcommand{\NineThreeSym}{9_{3}}
\newcommand{\NineThirtyVert}{585}
\newcommand{\NineThirtySym}{9_{30}}
\newcommand{\NineThirtyoneVert}{400}
\newcommand{\NineThirtyoneSym}{9_{31}}
\newcommand{\NineThirtytwoVert}{582}
\newcommand{\NineThirtytwoSym}{9_{32}}
\newcommand{\NineThirtythreeVert}{408}
\newcommand{\NineThirtythreeSym}{9_{33}}
\newcommand{\NineThirtyfourVert}{408}
\newcommand{\NineThirtyfourSym}{9_{34}}
\newcommand{\NineThirtyfiveVert}{566}
\newcommand{\NineThirtyfiveSym}{9_{35}}
\newcommand{\NineThirtysixVert}{579}
\newcommand{\NineThirtysixSym}{9_{36}}
\newcommand{\NineThirtysevenVert}{582}
\newcommand{\NineThirtysevenSym}{9_{37}}
\newcommand{\NineThirtyeightVert}{584}
\newcommand{\NineThirtyeightSym}{9_{38}}
\newcommand{\NineThirtynineVert}{585}
\newcommand{\NineThirtynineSym}{9_{39}}
\newcommand{\NineFourOneVert}{400}
\newcommand{\NineFourOneSym}{9^{4}_{1}}
\newcommand{\NineFourVert}{560}
\newcommand{\NineFourSym}{9_{4}}
\newcommand{\NineFortyVert}{583}
\newcommand{\NineFortySym}{9_{40}}
\newcommand{\NineFortyoneVert}{400}
\newcommand{\NineFortyoneSym}{9_{41}}
\newcommand{\NineFortytwoVert}{497}
\newcommand{\NineFortytwoSym}{9_{42}}
\newcommand{\NineFortythreeVert}{512}
\newcommand{\NineFortythreeSym}{9_{43}}
\newcommand{\NineFortyfourVert}{512}
\newcommand{\NineFortyfourSym}{9_{44}}
\newcommand{\NineFortyfiveVert}{535}
\newcommand{\NineFortyfiveSym}{9_{45}}
\newcommand{\NineFortysixVert}{490}
\newcommand{\NineFortysixSym}{9_{46}}
\newcommand{\NineFortysevenVert}{368}
\newcommand{\NineFortysevenSym}{9_{47}}
\newcommand{\NineFortyeightVert}{368}
\newcommand{\NineFortyeightSym}{9_{48}}
\newcommand{\NineFortynineVert}{368}
\newcommand{\NineFortynineSym}{9_{49}}
\newcommand{\NineFiveVert}{570}
\newcommand{\NineFiveSym}{9_{5}}
\newcommand{\NineSixVert}{400}
\newcommand{\NineSixSym}{9_{6}}
\newcommand{\NineSevenVert}{576}
\newcommand{\NineSevenSym}{9_{7}}
\newcommand{\NineEightVert}{575}
\newcommand{\NineEightSym}{9_{8}}
\newcommand{\NineNineVert}{571}
\newcommand{\NineNineSym}{9_{9}}

